Survey of different Large Language Model Architectures: Trends, Benchmarks, and Challenges

Large Language Models (LLMs) represent a class of deep learning models adept at understanding natural language and generating coherent responses to various prompts or queries. These models far exceed the complexity of conventional neural networks, often encompassing dozens of neural network layers and containing billions to trillions of parameters. They are typically trained on vast datasets, utilizing architectures based on transformer blocks. Present-day LLMs are multi-functional, capable of performing a range of tasks from text generation and language translation to question answering, as well as code generation and analysis. An advanced subset of these models, known as Multimodal Large Language Models (MLLMs), extends LLM capabilities to process and interpret multiple data modalities, including images, audio, and video. This enhancement empowers MLLMs with capabilities like video editing, image comprehension, and captioning for visual content. This survey provides a comprehensive overview of the recent advancements in LLMs. We begin by tracing the evolution of LLMs and subsequently delve into the advent and nuances of MLLMs. We analyze emerging state-of-the-art MLLMs, exploring their technical features, strengths, and limitations. Additionally, we present a comparative analysis of these models and discuss their challenges, potential limitations, and prospects for future development.

==> sections/bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{diagrams/authors/author1.png}}]{Minghao Shao} received the B.S. degree in Computer Science with Artificial Intelligence from University of Nottingham (UoN), United Kingdom, in 2020 and received M.S. degree in Computer Science from New York University (NYU), United States, in 2023. 
He is a Computer Science Ph.D. student co-advised by Prof. Muhammad Shafique at New York University Abu Dhabi (NYUAD) and Prof. Ramesh Karri at New York University Tandon School of Engineering. 
His research interests include Agent System for cybersecurity, Machine Learning Security, Model Compression and Efficient Inference for large language models and deep neural networks.
\end{IEEEbiography}

\vspace{-20pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{diagrams/authors/author2.png}}]{Abdul Basit} received the B.S. degree in electrical engineering from
the National University of Sciences and Technology (NUST), Pakistan, in 2021. Since August 2023, he has been with New York University Abu Dhabi (NYUAD), where he is currently a Research Engineer in the eBrain Laboratory. His research interests include autonomous driving, large language models, robotic systems, and security of face recognition models. He has been awarded the Rector's Gold Medal in B.S. EE. 

\end{IEEEbiography}
\vspace{-20pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{diagrams/authors/author3.png}}]{Ramesh Karri} (Fellow, IEEE) received the B.E. degree in electrical and computer engineering from Andhra University and the Ph.D. degree in computer science from the University of California San
Diego. He is currently a Professor of electrical and
computer engineering with New York University
(NYU) Tandon School of Engineering. He co-directs
the NYU Center for Cyber Security, co-founded
the Trust Hub, and founded the Embedded Systems
Challenge, the Annual Red Team Blue Team Event.
He has published over 300 articles in leading journals and conference proceedings. His research and education in hardware cybersecurity include trustworthy ICs, processors, and cyber-physical systems; security-aware computer-aided design, test, verification, and nano meets security; hardware security competitions, benchmarks, and metrics; and additive manufacturing security.
\end{IEEEbiography}
\vspace{-20pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{diagrams/authors/author4.png}}]{MUHAMMAD SHAFIQUE} (Senior Member, IEEE) received the Ph.D. degree in computer science from Karlsruhe Institute of Technology, Karlsruhe, Germany, in 2011. He was a Full Professor at the Institute of Computer Engineering, TU Wien, Vienna, Austria, from October 2016 to August 2020. Since September 2020, he has been with the Division of Engineering, New York University Abu Dhabi, Abu Dhabi, UAE, and is a Global Network Faculty Member of the NYU Tandon School of Engineering, Brooklyn, NY, USA. His research interests are in system-level design for brain-inspired computing, AI/machine learning hardware, wearables, autonomous systems, energy-efficient and robust computing, IoT, and smart CPS. Dr. Shafique received the 2015 ACM/SIGDA Outstanding New Faculty Award, the AI 2000 Chip Technology Most Influential Scholar Award in 2020, 2022, and 2023, six gold medals, and several best paper
awards and nominations. He has given several keynotes, talks, and tutorials and organized special sessions at premier venues. He has served as the PC chair, general chair, track chair, and PC member for several conferences.

% (Senior Member, IEEE) received the Ph.D. degree in computer science from the Karlsruhe Institute of Technology (KIT), Germany, in 2011. Afterwards, he established and led a highly recognized research group with KIT for several years as well as conducted impactful collaborative research and development activities across the globe. In October 2016, he joined the Institute of Computer Engineering, Faculty of Informatics, Technische Universität Wien (TU Wien), Vienna, Austria, as a Full Professor of computer architecture and robust energy-efficient technologies. Since September 2020, he has been with New York University (NYU), where he is currently a Full Professor and the Director of the eBrain Laboratory, NYU Abu Dhabi (NYUAD), United Arab Emirates, and a Global Network Professor with the Tandon School of Engineering, NYU New York City, USA. He is also a Co-PI/Investigator in multiple NYUAD centers, including the Center of Artificial Intelligence and Robotics (CAIR), the Center of Cyber Security (CCS), the Center for InTeractIng urban nEtworkS (CITIES), and the Center for Quantum and Topological Systems (CQTS). He holds one U.S. patent. He has (co)authored six books, more than ten book chapters, more than 350 papers in premier journals and conferences, and more than 100 archive articles. His research interests include AI and machine learning hardware and system-level design, brain-inspired computing, machine learning security and privacy, quantum machine learning, cognitive autonomous systems, wearable healthcare, energy-efficient systems, robust computing, hardware security, emerging technologies, FPGAs, MPSoCs, and embedded systems. His research has a special focus on cross-layer analysis, modeling, design, and optimization of computing and memory systems. The researched technologies and tools are deployed in application use cases from the Internet of Things (IoT), smart cyber-physical systems (CPS), and ICT for development (ICT4D) domains. He is a Senior Member of the IEEE Signal Processing Society (SPS) and a member of the ACM, SIGARCH, SIGDA, SIGBED, and HIPEAC. He received the 2015 ACM/SIGDA Outstanding New Faculty Award, the AI 2000 Chip Technology Most Influential Scholar Award, in 2020 and 2022, the 2015 ACM/SIGDA Outstanding New Faculty Award, the AI 2000 Chip Technology Most Influential Scholar Award, in 2020, 2022, and 2023, the ASPIRE AARE Research Excellence Award, in 2021, six gold medals, and several best paper awards and nominations at prestigious conferences. He has served as the PC chair, the general chair, the track chair, and a PC member for several prestigious IEEE/ACM conferences. He has given several keynotes, invited talks, and tutorials, as well as organized many special sessions at premier venues. VOLUME 12, 2024 1
\end{IEEEbiography}

==> sections/draft.tex <==
\section{Development of Large Language Models}
In this section, we would have a brief overview on the development of large language model. Most of the modern LLM was designed based on Transformer, which was proposed in the year 2017 [], hence in this section, we would have a detailed timeline based on the year 2017 and introduce some of the capstone models in the development of LLM in chronological order.

\subsection{Year 2017 - Transformer}
Vaswani et al. originally developed The Transformer, a deep learning architecture, in 2017 for sequence-to-sequence learning applications including text summarization and machine translation. The Transformer substitutes the sequential processing of input tokens with a self-attention mechanism that enables the model to attend to all input tokens concurrently, in contrast to conventional recurrent neural network (RNN) based techniques. In order to calculate a weighted sum of the input tokens, the self-attention mechanism computes attention weights between each input token and each token in the sequence.
Transformer was organised in Encoder-Decoder architecture, using self-attention and feedforward layers, the encoder computes a collection of hidden representations from an input sequence. Using the output of the encoder as input, the decoder creates the output sequence one token at a time, conditionally depending on the tokens that came before and the output of the encoder.
On a variety of natural language processing tasks, such as machine translation, text summarization, question answering, and language modeling, The Transformer has attained cutting-edge performance. Additionally, the Transformer served as the foundation for a number of substantial language models, including GPT, BERT, and T5, all of which have helped to advance the state-of-the-art in NLP.

\subsection{Year 2018}
Large language models (LLMs) for natural language processing made major advancements in 2018. OpenAI launched GPT, a language model that performed well on a range of language tasks. BERT, a newly published iteration of Google's language model, surpassed earlier iterations on a number of metrics. Researchers also looked at adaptive gradient techniques and neural architecture search for training and optimizing LLMs. Overall, LLM development and optimization made considerable strides in 2018, and these developments are what continue to propel NLP forward.

\subsubsection{GPT-1}
Large language model GPT-1, or the Generative Pre-trained Transformer, was created by OpenAI and published in June 2018. Using a self-supervised pre-training technique, the model is trained on a vast corpus of text, comprising web pages, books, and other sources. A transformer-based encoder-decoder architecture with 12 transformer blocks, 117 million parameters, and a maximum sequence length of 512 tokens makes up the GPT-1 architecture. A masked language modeling aim was used to train the model, which predicts the original token based on context by masking a random subset of input tokens.
According to experimental findings, GPT-1 performed at the cutting edge on a number of language tasks, including text completion, question-answering, and language modeling. Additionally, the model showed outstanding text production abilities, producing cohesive and fluid language across a range of genres, including poetry and news pieces. GPT-1 still had significant drawbacks, such as the requirement for a lot of training data and sometimes repetitious or unintelligible replies. Overall, GPT-1 laid the ground for later developments in natural language processing and represented an important turning point in the creation of huge language models.

\subsubsection{BERT}
In October 2018, Google unveiled BERT, or Bidirectional Encoder Representations from Transformers, a sizable pre-trained language model. The model is trained using a mix of masked language modeling and next sentence prediction targets on a substantial corpus of text, including books, journals, and online pages. A transformer-based encoder that can be customized for a variety of natural language processing applications is the foundation of the BERT architecture. BERT-base and BERT-large, two variations of the model, include 110 million and 340 million parameters, respectively.
According to experimental findings, BERT performed at the cutting edge on a number of natural language processing tasks, including sentiment analysis, question answering, and natural language inference. Due to the model's ability to gather contextual information from both the left and right sides of a given token, it performed noticeably better than earlier models. Furthermore, BERT's fine-tuning strategy made it simple to adapt to a variety of tasks with only modest quantities of task-specific data. In terms of big pre-trained language models, BERT was a significant step forward and has subsequently been the foundation for many other models and applications.

\subsubsection{mBERT}
A large pre-trained language model called mBERT, or Multilingual BERT, was created by Google in November 2019. Instead of developing distinct models for each language, mBERT aims to construct a single language model that can handle numerous languages. By training on a vast corpus of text in several languages, including books, articles, and web pages, mBERT does this. The design of the model is based on BERT, but it also includes a language embedding layer to support many languages. There are two types of mBERT: mBERT-base and mBERT-large, each containing 110 million and 340 million parameters.
mBERT was trained using the same masked language modeling and next sentence prediction goals as BERT on a sizable corpus of text from more than 100 different languages. The model has a transformer-based design, like BERT, and includes 110 million parameters. According to experimental findings, mBERT performed impressively on a number of cross-lingual natural language processing tasks, including named entity identification, part-of-speech tagging, and sentence categorization. The model also displayed zero-shot cross-lingual transfer, or the capacity to generalize to languages it has not specifically been trained on. Overall, mBERT represents a substantial advancement in the creation of large pre-trained language models and has important ramifications for the multilingual NLP community.


\subsubsection{MultiFIT}
The language model fine-tuning approach known as MultiFIT, or Efficient Multi-lingual Language Model Fine-tuning, permits effective training of large-scale multilingual models on a variety of languages. It was released in 2019. MultiFIT's goal is to decrease the computational expense and training time necessary for fine-tuning multilingual models on a new language while preserving or enhancing performance in comparison to conventional fine-tuning techniques. MultiFIT is built on the straightforward yet powerful concept of multi-task learning, in which a model is concurrently trained for a number of related tasks. The authors provide a cutting-edge training method that takes use of the commonalities between several languages in order to train a multilingual model on a variety of tasks in a single run. For example, they employ a task-specific loss function that considers the language ID of each input character, enabling the model to successfully identify across languages and modify its representations.
According to experimental findings, MultiFIT performed at the cutting edge on a number of multilingual natural language processing tasks, including part-of-speech tagging, named entity identification, and cross-lingual document categorization. Comparing the model to conventional fine-tuning techniques, it also showed notable gains in productivity and training time. Overall, MultiFIT is a substantial advancement in the creation of multilingual language models with important ramifications for the multilingual NLP community.

\subsubsection{LXMERT}
In order to complete a variety of tasks, including visual question-and-answer processing and visual reasoning, the LXMERT large-scale, multimodal language model mixes linguistic and visual data. It was created by UNC Chapel Hill academics and made public in August 2019. By allowing the model to reason simultaneously about both modalities using a common semantic space that captures their interactions, LXMERT aims to close the gap between language and vision. Using a multi-task learning architecture, LXMERT is trained on a substantial corpus of text and pictures from the COCO and Visual Genome datasets. These datasets include masked language modeling, image captioning, and visual question answering. The model comprises of a joint embedding module that unifies the two modalities after a transformer-based design that integrates text and picture encoders. The resultant model is capable of a variety of tasks, including responding to inquiries in plain language regarding images, creating captions for images, and resolving visual reasoning conundrums.
The findings of the experiments demonstrated that LXMERT outperformed earlier models that relied only on language or visual input to execute, achieving state-of-the-art performance on a number of multimodal natural language processing tasks, including visual question answering and visual reasoning. The model also showed that it could generalize to new tasks and domains without more training, a process known as zero-shot transfer. LXMERT is a significant advancement in the creation of multimodal language models overall, with important ramifications for the multimodal natural language processing community.

\subsubsection{VideoBERT}
A multimodal language model called VideoBERT is capable of learning joint representations of both linguistic and visual data. It was created by Google AI researchers and launched in April 2019. With the use of VideoBERT, a model will be able to comprehend the semantic connections between video and linguistic information and provide natural language descriptions of video content.
A transformer-based architecture that integrates video and language encoders, followed by a joint embedding module that unifies the two modalities, is used to train VideoBERT on a sizable corpus of video and language data. The model is trained on a multi-task goal that consists of visual-semantic embedding, video captioning, and masked language modeling. The model that emerges is capable of carrying out a number of tasks, including producing natural language descriptions of films, responding to natural language inquiries about videos, and carrying out video retrieval based on natural language queries. The usefulness of combined learning of video and language data was demonstrated by experimental findings showing that VideoBERT surpassed earlier models on a number of video and language tasks.

\subsection{Year 2019}
LLM development went further in 2019 with a focus on advancements in fields including reinforcement learning, computer vision, and natural language processing (NLP). With the emergence of transformer models like BERT and GPT-2, which significantly enhanced language understanding and generating capabilities, significant advancements in NLP were made. With the development of increasingly complex convolutional neural networks, computer vision also made great strides, while reinforcement learning gained ground with applications in robotics and gaming. The ethical issues surrounding the use of LLMs, notably those relating to prejudice and impartiality, were also given more attention.

\subsubsection{Transformer-XL}
Transformer-XL is a language model that was introduced by researchers at Carnegie Mellon University and Google AI in January 2019. The objective of Transformer-XL is to address the problem of limited context modeling in existing transformer-based language models, which typically only consider a fixed length of preceding context. To achieve this, Transformer-XL uses a novel architecture that allows for the dynamic computation of contextual representations of varying lengths.
Using an autoregressive language modeling aim, Transformer-XL is trained on a sizable corpus of text with a focus on capturing long-term relationships in language data. Long-term dependencies may be captured by the model without losing computational speed thanks to a relative positional encoding method and a segment-level recurrence mechanism in the model design. Transformer-XL surpassed current state-of-the-art models, according to experimental results on a number of language modeling benchmarks, particularly on tasks that call for the modeling of long-range dependencies, such language interpretation and creation.

\subsubsection{GPT-2}
GPT-2 was created by OpenAI and launched in February 2019. By creating a model that could produce cohesive, high-quality text with little to no fine-tuning, GPT-2 aimed to advance the state-of-the-art in language modeling. One of GPT-2's key advances is its capacity to produce lengthy, cohesive texts that are identical to those authored by humans.
Web pages, books, and articles were all included in the large text dataset used to train the GPT-2 algorithm. After preprocessing and tokenizing the dataset with byte pair encoding, a vocabulary of 50,257 subword units was produced. One of the biggest language models ever created, GPT-2 has a transformer design with 12 transformer blocks and 117 million parameters. GPT-2 surpassed current state-of-the-art models by a large margin, especially on tasks that call for the creation of cohesive and high-quality text, according to experimental results on multiple language modeling benchmarks.

\subsubsection{CTRL}
A language model called CTRL (Conditional Transformer Language Model for Controllable Generation) was created to enable users to manage the style, content, and duration of generated text. A conditional training approach is used by the model, which is based on the Transformer architecture and enables fine-grained control over the output created. Use of a customizable latent code, which enables users to specify the desired properties of the produced text, is the main novelty of CTRL.
A group of academics from Salesforce Research, the University of California, Berkeley, and the University of Montreal unveiled CTRL in February 2019. A broad selection of 3,000 books totaling 45GB in size, comprising fiction, non-fiction, and scientific material, were used to train the model. The CTRL design includes a decoder-only Transformer with a causal self-attention mechanism and a cutting-edge method for discovering the hidden code that permits controlled creation. On a number of language creation tasks, including as creating Wikipedia articles, stories, and code from natural language, the model demonstrated state-of-the-art performance.

\subsubsection{Megatron}
Researchers at NVIDIA created the language model known as Megatron-LM, which enables the model parallelism training of multi-billion parameter models. In order to increase performance on a variety of natural language processing tasks, this effort aims to scale up language models to collect additional contextual data. Since its September 2019 debut, Megatron-LM has produced cutting-edge performance across a range of benchmarks.
The transformer architecture serves as the foundation for Megatron-LM's architecture, which is built to facilitate effective model parallelism. Due to the model parallelism, very large models may be trained utilizing distributed compute across several GPUs. In order to decrease the amount of memory needed to train huge models, the researchers used a hybrid parallelism approach and gradient accumulation, among other strategies, to optimize the training process. Megatron-LM was trained using 8.3 billion tokens of text data from a variety of sources, including Wikipedia, online pages, novels, and scientific publications. The outcomes of the experiment demonstrate that Megatron-LM performs at a state-of-the-art level on a variety of language modeling benchmarks, including WikiText-103, One Billion Words, and LAMBADA, and also enhances its performance on downstream NLP tasks, including sentiment analysis, question answering, and summarization.

\subsubsection{XLNet}
Yang et al.'s 2019 proposal for XLNet is a generalized autoregressive pretraining language model. By tackling the problem of information loss during pretraining, XLNet seeks to overcome the drawbacks of earlier language models like BERT. The idea of "permutation language modeling," which XLNet provides, enables the model to take into account all conceivable permutations of the input sequence during training. In order to do this, a generalized autoregressive objective function is used, which is based on all potential permutations of the input sequence's tokens. XLNet can capture more intricate links between the tokens in the input sequence by taking into account all potential permutations.
The English Wikipedia and BookCorpus were two of the several text corpora used to train the model. With the inclusion of two-stream self-attention, relative positional encoding, and a segment recurrence mechanism, XLNet utilizes a similar architecture to that of the transformer. According to experimental findings, XLNet beats earlier state-of-the-art models on a variety of natural language processing tasks, such as sentiment analysis, question answering, and natural language inference.

\subsubsection{UnitLM}
UniLM, pre-trains a single model to perform a variety of natural language processing tasks, including comprehending and producing natural language. Microsoft Research put out UniLM in 2019 as a step toward creating a single model that is capable of handling a variety of NLP tasks. The fundamental advancement in UniLM is the use of a multi-task learning goal, which enables the model to be trained on several tasks at once and learn common representations across them. With less labeled data available, this results in higher performance on downstream tasks. A vast corpus of text data is utilized to pre-train UniLM, which is then used to learn broad language representations that may be tailored for particular purposes.
Over 16GB of text data from sources including the English Wikipedia, BookCorpus, and a web corpus were used to train UniLM. Similar to other cutting-edge language models, UniLM's model architecture is built on the Transformer architecture. Several natural language processing tasks, including machine translation, text categorization, and text creation, were completed by UniLM with state-of-the-art results, illuminating the potency of the multi-task learning strategy employed by UniLM.

\subsubsection{ERNIE}
Researchers at Baidu created the natural language processing paradigm known as ERNIE (Enhanced Representation via Knowledge IntEgration). The goal of ERNIE is to enhance language representation and comprehension by fusing data from multiple sources. ERNIE, which was introduced in May 2019, was created to overcome some of the shortcomings of current language models, specifically their lack of comprehension of context and real-world information.
Chinese language text, English language text, and structured knowledge bases like Wikipedia and Baidu Baike are just a few of the enormous datasets used to train ERNIE. By adding factual and contextual information, this helps the model to more fully comprehend the subtleties and intricacies of language. An entity-aware encoding scheme and a knowledge masking strategy are only two of the cutting-edge methods that ERNIE uses to further improve the model's capacity for understanding and reasoning with data. According to experimental findings, ERNIE performs at the cutting edge on a variety of tasks involving the interpretation and creation of natural language, such as sentiment analysis, named entity identification, and machine translation. The model has also shown promise in overcoming some of the drawbacks of conventional language models, specifically their inability to integrate information.

\subsubsection{ALBERT}
A self-supervised learning approach called ALBERT, sometimes known as A Lite BERT, is used to train language representations. It was first mentioned by Zhenzhong Lan et al. from Google Research and the Toyota Technological Institute in Chicago in a report published in 2019. ALBERT's main goal is to attain accuracy on par with or better than BERT while using fewer parameters and more effectively using computing resources.
Two novel training methods were used to train ALBERT on a large amount of text data: (1) factorized embedding parameterization, which lowers the number of parameters in the embedding layer, and (2) cross-layer parameter sharing, which allows parameters to be shared between layers of the neural network. As a result, ALBERT may be trained with less parameters than BERT and yet perform as well as or better than BERT on a variety of natural language processing tasks, including sentiment analysis and question answering. According to the experimental findings, ALBERT beats BERT in terms of the quantity of parameters and training efficiency, while also reaching parity or superior accuracy on a variety of language understanding tasks.

\subsubsection{VL-BERT}
A pre-trained language model called VL-BERT enables the learning of integrated representations of both visual and verbal input. Researchers from Microsoft and the University of Science and Technology of China first presented it in 2019. The model aims to capture the intricate links between words and visuals in order to improve the capacity of natural language processing. VL-BERT's employment of an attention mechanism that can simultaneously attend to visual and textual inputs is what makes it novel. This attention technique enables the model to simultaneously capture the matching visual characteristics and encode the context of the textual input.
The model was pre-trained on the Conceptual Captions dataset, which contains over 3 million image and caption pairs. The training process involved a combination of two pre-training objectives: masked language modeling and image-text matching. The architecture of VL-BERT is based on the Transformer model, with the addition of a visual embedding layer that maps the input image to a shared embedding space with the textual data. According to experimental findings, VL-BERT performs better than cutting-edge techniques in a number of downstream tasks, including picture captioning, answering visual questions, and understanding referring expressions. Additionally, VL-BERT has demonstrated to be very effective in multi-task learning settings, allowing the model to be modified on several tasks at once. These findings highlight the efficiency of VL-BERT in learning combined representations of visual and linguistic input as well as its potential for a range of uses in computer vision and natural language processing.

\subsubsection{LayoutML}
A pre-trained model for document image comprehension called LayoutLM can concurrently detect a document picture's textual content and layout structure. Researchers from Microsoft Research Asia and the Harbin Institute of Technology came up with the idea. By utilizing the layout data, LayoutLM seeks to enhance the efficiency of information extraction from document photos. 
A sizable corpus of document pictures and the related OCR (Optical Character Recognition) outputs served as the basis for LayoutLM's pre-training. A standard masked language modeling objective is used in the first stage of the pre-training process, which consists of two stages. In the second stage, a novel masked layout modeling objective is used to pre-train the model on both textual and layout information. A well-known deep learning model for natural language processing, the Transformer, serves as the foundation for LayoutLM's model architecture. Studies on a variety of downstream tasks, including information extraction, problem-solving, and table recognition, have revealed that LayoutLM performs noticeably better than earlier state-of-the-art approaches.

\subsubsection{BART}
Modern denoising sequence-to-sequence pre-training technique for natural language synthesis, translation, and comprehension is called BART (Bidirectional and Auto-Regressive Transformer). A group of researchers from Facebook AI Research (FAIR) came up with BART in 2019. BART's goal is to provide a pre-training method that can acquire reliable language representations for a variety of downstream tasks by figuring out how to restore damaged text.
BART's ability to integrate bidirectional and auto-regressive training in a single design is its main breakthrough. By mastering the skill of denoising distorted input sequences, the model is trained on a wide variety of tasks, such as machine translation, summarization, and question answering. The BookCorpus and the English Wikipedia were used to train BART, which has now demonstrated state-of-the-art performance on a number of benchmark datasets for a variety of NLP tasks.
BART has demonstrated cutting-edge performance in experimental assessments on a range of language creation and comprehension tasks, including machine translation, summarization, and question answering. The architecture of the model enables bidirectional and auto-regressive learning, which makes it suitable for both encoding and decoding applications. On a number of benchmark datasets, BART's performance has been proven to be superior to that of earlier state-of-the-art models, such as GPT-2 and T5, proving its capacity to acquire reliable and adaptable language representations. Since its debut, BART has significantly improved natural language processing, making it a crucial tool for academics and industry professionals.

\subsubsection{ViLBERT}
The state-of-the-art pre-training approach ViLBERT (Vision-and-Language BERT) creates task-independent visio-linguistic representations for a variety of vision-and-language tasks, including picture captioning, visual question answering, and visual entailment. A group of academics from Oregon State University, Georgia Institute of Technology, and Facebook AI Research (FAIR) came up with the idea for ViLBERT in 2019. By pre-training on a substantial corpus of text and pictures, the basic goal of ViLBERT is to acquire combined representations of visual and linguistic data that may subsequently be refined on particular tasks involving vision and language.
ViLBERT's use of a multi-modal transformer architecture, which combines both language and visual input and enables the model to concurrently reason about both modalities, is its fundamental novelty. ViLBERT is trained using two pre-training tasks: masked multimodal modeling and visual-linguistic matching, using a huge corpus of text and images, including the Conceptual Captions and Visual Genome datasets. ViLBERT surpasses earlier state-of-the-art models in experimental assessments on a variety of vision-and-language tasks, including visual entailment and VQA, proving the viability of its joint representation learning methodology.
ViLBERT has demonstrated cutting-edge performance in experimental assessments on a variety of vision-and-language tasks, including picture captioning, visual question answering, and visual entailment. The model can successfully reason about both modalities because to the design that enables it to learn combined representations of visual and language data. On several benchmark datasets, ViLBERT has been shown to outperform previous state-of-the-art models, such as BERT and the bottom-up/top-down attention model, proving its capacity to learn task-independent visio-linguistic representations that are helpful for a variety of vision- and language-related tasks. Since its debut, ViLBERT has significantly advanced the study of vision-and-language comprehension, making it an indispensable tool for academics and professionals working on a range of vision-and-language activities.

\subsection{Year 2020}
With significant developments in areas including natural language processing, computer vision, and generative modeling, the development of LLMs accelerated in 2020. The GPT-3 language model, the largest and most potent language model at the moment, was one of the capstone models that was revealed. It is capable of producing coherent and context-aware answers to a variety of natural language challenges. The T5 model, which provided a consistent framework for several NLP tasks including summarization, translation, and question-answering, was another important one. The GAN-based models StyleGAN2 and BigGAN enhanced picture synthesis and manipulation, while the DALL-E model, which can produce images from textual descriptions, was presented in generative modeling.

\subsubsection{Turing-NLG}
One of the biggest language models ever made, Turing-NLG is a cutting-edge language model designed by Microsoft that has 17 billion parameters. The model, which was introduced in February 2020, can produce excellent text in several other languages, including English, Chinese, French, and German. By pushing the limits of language modeling to an unprecedented size and quality, Turing-NLG aims to enhance natural language understanding and generation.
Turing-NLG's large-scale design, which enables the model to capture intricate linguistic patterns and produce high-quality text in several languages, is its fundamental breakthrough. The model is trained using a combination of supervised and unsupervised learning methods on a sizable corpus of text data, including web pages, books, and news items. Turing-NLG's large-scale design has been shown successful by experimental tests showing that it beats earlier state-of-the-art models on a variety of natural language processing tasks, such as language modeling, text categorization, and question answering.
Turing-NLG has demonstrated cutting-edge performance in experimental assessments on a variety of language modeling and natural language processing tasks, including the SuperGLUE benchmark for natural language comprehension and the LAMBADA benchmark for language modeling. A useful tool for researchers and practitioners in the field of natural language processing, the model's large-scale design enables it to catch intricate linguistic patterns and produce high-quality text in several languages. The publication of Turing-NLG is an important development in the field of language modeling, showing the capacity of massive language models to produce excellent text and enhance natural language comprehension.

\subsubsection{OSCAR}
Oscar (Object-Semantics Aligned Pre-training for Vision-Language Tasks) was created by Microsoft to provide object-semantics aligned representations for diverse vision-and-language tasks. The approach, which was unveiled in April 2020, aims to increase comprehension of visual concepts by aligning object and word embeddings. By pre-training on a sizable corpus of text and pictures to acquire combined representations of visual and linguistic input, Oscar aims to improve the performance of vision-and-language tasks.
Oscar's use of a multi-modal transformer architecture, which aligns word and object embeddings and enables the model to comprehend visual ideas and their related verbal descriptions, is its fundamental innovation. The model is trained utilizing a variety of pre-training tasks, such as masked object-region modeling, masked word-region modeling, and image-text matching, using a huge corpus of text and pictures, including the Conceptual Captions and COCO datasets. Oscar's joint representation learning strategy has been shown to be effective by experimental results showing that it beats earlier state-of-the-art models on a variety of vision-and-language tasks, including as picture captioning, visual question answering, and visual entailment.
Oscar has demonstrated innovative performance in experimental assessments on a variety of vision-and-language tasks, including picture captioning, visual question answering, and visual entailment. The model's architecture enables alignment of object and word embeddings, which improves its comprehension of both written and visual concepts. The capacity of Oscar to learn object-semantics aligned representations that are helpful for a variety of vision-and-language tasks has been proven to outperform earlier state-of-the-art models, such as BERT and ViLBERT, on many benchmark datasets. Since its debut, Oscar has significantly advanced the study of vision-and-language comprehension, making it a crucial tool for academics and professionals working on a range of vision-and-language problems.

\subsubsection{ERNIE-2.0}
Baidu Research has created a continuous pre-training framework for language comprehension called ERNIE 2.0 (Enhanced Representation via kNowledge IntEgration 2.0). The concept, which was unveiled in July 2019, aims to incorporate expertise from several fields into the pre-training and fine-tuning procedures. With the help of knowledge integration from diverse sources and pre-training on massive amounts of text data, ERNIE 2.0 aims to increase language understanding across a variety of areas and languages.
The fundamental advancement of ERNIE 2.0 is its continuous pre-training architecture, which enables the model to include information from many domains, including knowledge graphs, question-answering datasets, and domain-specific corpora. Using a variety of pre-training tasks, such as masked language modeling, sentence-pair matching, and knowledge masking, the model is pre-trained on a vast corpus of text data, including web pages, news articles, and novels. ERNIE 2.0 outperforms earlier state-of-the-art models in experimental evaluations on a variety of natural language processing tasks, including sentiment analysis, named entity recognition, and question answering, proving the value of its continuous pre-training framework.
On a variety of natural language processing tasks in Chinese and English, including as sentiment analysis, named entity identification, and question answering, ERNIE 2.0 has demonstrated state-of-the-art performance in experimental assessments. The model can incorporate information from many domains thanks to its continuous pre-training architecture, which enhances its performance on numerous language understanding tasks. With the introduction of ERNIE 2.0, substantial progress has been made in the field of natural language processing, proving the value of using data from multiple sources in pre-training and fine-tuning procedures.

\subsubsection{RoBERTa}
2019 saw the launch of RoBERTa, an advanced pre-training method for problems involving natural language processing developed by the University of Washington and Facebook AI. Known as the "Robustly Optimized BERT Approach," the BERT (Bidirectional Encoder Representations from Transformers) model has been improved upon by RoBERTa. The main goal of RoBERTa is to enhance BERT's performance by enhancing its training procedure and hyperparameters, enabling the model to acquire more accurate language representations.
RoBERTa's optimized training method, which pre-trains on a substantial corpus of text data, including BookCorpus and English Wikipedia, employing a mix of pre-training tasks, including masked language modeling and next sentence prediction, is the main novelty of the system. By adjusting hyperparameters like the batch size, learning rate schedule, and number of training steps, RoBERTa's training procedure is made as efficient as possible. RoBERTa outperforms BERT and other cutting-edge models in experimental tests on a variety of natural language processing tasks, including sentiment analysis, question answering, and named entity recognition, proving the value of its optimized pre-training strategy.
RoBERTa has outperformed earlier state-of-the-art models like BERT and XLNet in experimental assessments, achieving cutting-edge performance on a variety of natural language processing tasks. The model performs better on a variety of language understanding tests because to its enhanced training method, which enables it to acquire better language representations. With the introduction of RoBERTa, tremendous progress has been made in the area of natural language processing, making it a crucial tool for academics and professionals working on a variety of language comprehension problems.

\subsubsection{ELECTRA}
A pre-training method for natural language processing problems called ELECTRA was announced in March 2020 by Stanford University and Google Brain researchers. The main novelty of ELECTRA is that it pre-trains text encoders using a discriminator model rather than a generator model, as in other pre-training techniques like BERT. Enhancing the efficacy and efficiency of pre-training for activities involving natural language processing is the goal of ELECTRA.
In order to discriminate between "real" and "fake" input sequences, the ELECTRA training procedure requires training a discriminator model. The "fake" sequences are produced by randomly changing certain tokens in the "real" sequences. The goal is to optimize the text encoder, which serves as the generator for these "fake" sequences, such that it can create "fake" sequences that are identical to the "real" ones. Because fewer calculations are needed to produce "fake" sequences, this method of pre-training is more effective than earlier methods. On a variety of natural language processing tasks, experimental assessments have shown that ELECTRA performs better than BERT and other cutting-edge pre-training techniques, proving the efficacy of its discriminator-based methodology.
Since ELECTRA provides a more effective pre-training method for text encoders, its introduction has significantly advanced the area of natural language processing. On a variety of language comprehension tasks, it has been demonstrated that its discriminator-based technique outperforms earlier generator-based systems, such as BERT. Due to this, it has become a crucial tool for practitioners and scholars engaged in a variety of natural language processing projects.

\subsubsection{Wav2vec 2.0}
In October 2020, Facebook AI researchers announced wav2vec 2.0, a framework for self-supervised learning for speech representations. Wav2vec 2.0's capacity to learn speech representations through contrastive learning without labeled input is by far its most significant improvement. The framework's objective is to boost the effectiveness and efficiency of voice recognition and other speech-based tasks.
A pre-training stage and a fine-tuning stage are the two primary phases of the wav2vec 2.0 training process. The framework is trained on a sizable corpus of unlabeled speech data during the pre-training step in order to develop a set of useful speech representations. The framework is taught to differentiate between "positive" and "negative" instances of voice data using a contrastive learning technique. The pre-trained model is adjusted at the fine-tuning step for a particular speech-related task, such as voice recognition or speaker recognition, using a smaller labeled dataset. On a variety of speech-related tasks, experimental assessments have shown that wav2vec 2.0 outperforms earlier state-of-the-art speech representation learning frameworks, proving the viability of its contrastive learning strategy.
The release of wav2vec 2.0 has significantly improved speech recognition and other speech-related tasks since it provides a more effective method of learning voice representations without any labeled input. On a variety of speech-related tasks, it has been demonstrated that its contrastive learning technique performs better than earlier unsupervised and supervised learning systems. As a result, it has become a crucial tool for academics and professionals working on voice recognition and other activities involving speech.

\subsubsection{UNITER}
A universal image-text representation learning system called UNITER was launched by researchers from Microsoft Dynamics 365 AI Research in July 2020 with the goal of bridging the gap between vision and language. The framework's goal is to provide a combined representation space for text and pictures that may be used to tackle a variety of image-text tasks, including image captioning and answering visual questions.
A transformer-based architecture is used by UNITER to enable it to learn a shared representation space for both pictures and text. A big image-text corpus with more than 2.8 million image-text pairs from diverse sources served as the framework's pre-training data. By utilizing a multi-modal transformer architecture during pre-training, the framework learns to connect pictures and text in a shared embedding space. The pre-trained model may then be adjusted for use in certain picture-text tasks, including image captioning and answering visual questions. On a variety of image-text tasks, experimental assessments have shown that UNITER performs better than prior state-of-the-art systems, proving the viability of its joint representation learning strategy.
Since UNITER provides a more efficient method of learning a joint representation space for both pictures and text, it has significantly advanced the area of image-text representation learning. It has been demonstrated that its transformer-based design and multi-modal pre-training approach outperform earlier approaches on a variety of image-text tasks, making it a crucial tool for practitioners and researchers working on image-text tasks.

\subsubsection{T5}
Researchers from Google AI released a study titled "Exploring the Limits of Transfer Learning with a Unified Text-to-Text Transformer (T5)" in July 2020. With a unified text-to-text transformer model, the goal of this work is to investigate the boundaries of transfer learning. The main advancement of T5 is its ability to train on a variety of natural language processing (NLP) tasks, from text categorization to question answering, utilizing a single architecture and pre-training procedure.
A sizable quantity of data from several sources, including books, online pages, and Wikipedia articles is used to train the T5 model. Using a transformer-based architecture, the model gains the ability to create an output sequence from an input sequence during pre-training. The pre-trained model may then be improved for use in a variety of downstream NLP tasks, including question answering, summarizing, and language modeling. The experimental findings of T5 demonstrate the efficacy of its unified transfer learning strategy by showing that it beats earlier state-of-the-art models on a variety of NLP tasks. Because T5 provides a more efficient method of carrying out transfer learning for a variety of NLP tasks, it has significantly advanced the discipline of NLP.

\subsubsection{GPT-3}
Modern natural language processing model GPT-3 (Generative Pre-trained Transformer 3) was created by OpenAI. It was released in June 2020 and has 175 billion parameters, more than 10 times as many as its predecessor, GPT-2, making it the biggest language model in existence. The main goal of GPT-3 is to produce text that reads coherently and human-like by foretelling the most likely next word in a given text sequence. Contrary to its forerunners, GPT-3 can carry out a variety of natural language processing tasks with high accuracy and little fine-tuning, including machine translation, question-answering, text completion, and summarization.
The unique feature of GPT-3 is its capacity for few-shot learning, which allows it to pick up a new skill with a small number of training samples. This is accomplished by adopting a cutting-edge technique called prompt-based learning, in which the model is provided with a prompt that details the job it must complete along with a few examples. These examples are used by GPT-3 to produce coherent output for the assigned task. GPT-3 achieves state-of-the-art performance on a number of benchmark datasets thanks to training it on a sizable corpus of web pages known as the Common Crawl and fine-tuning it for a variety of natural language processing tasks. With potential uses in chatbots, virtual assistants, and other language-based artificial intelligence systems, it is a significant milestone in the field of natural language processing thanks to its outstanding performance and few-shot learning capabilities. With potential uses in chatbots, virtual assistants, and other language-based artificial intelligence systems, it is a significant milestone in the field of natural language processing thanks to its outstanding performance and few-shot learning capabilities.

\subsubsection{GShard}
Google Research has introduced GShard as a new method for scalability of deep learning models. The main novelty of GShard is the use of autonomous sharding and conditional computing to enable the training of very large models, such as the trillion-parameter models that are anticipated to be required for future AI applications. With communication between the sub-models, GShard accomplishes this scalability by breaking a model down into smaller sub-models that may be trained separately and concurrently. A cutting-edge hierarchical attention mechanism is also incorporated into GShard to facilitate effective communication and computation amongst the sub-models.
The document was written by a group of Google Research experts and published on arXiv in June 2020. As the emphasis is on the architecture and methods used to enable scaling rather than on particular applications, the training set used to test GShard is not disclosed in the study. In comparison to other methods for scaling up deep learning models, the experimental findings show that GShard is capable of achieving appreciable speedups and increased efficiency, making it a potential strategy for creating even bigger and more potent models in the future.

\subsubsection{Virtex}
A visual pre-training model called VirTex learns superior visual characteristics from annotated text. Researchers from the University of Michigan made the suggestion. The lack of annotated visual data, which complicates many visual recognition tasks, is a problem that VirTex seeks to address. The model can learn visual characteristics from textual descriptions since it was trained on a vast number of unannotated photos and annotations.
It was released in September 2021, was trained using both private and public Facebook image descriptions. Encoder and decoder, both of which are transformer-based, make up VirTex's architecture. The decoder is used to provide visual features, while the encoder analyzes the incoming textual annotations. A contrastive objective function is used to train the model, which pushes the encoder to provide comparable representations for semantically related annotations. VirTex demonstrated its capacity to acquire superior visual characteristics from textual annotations by achieving state-of-the-art results on a variety of visual recognition tasks, including picture categorization, object identification, and visual question answering.

\subsubsection{ProphetNet}
In 2020, researchers from Microsoft, University of Science and Technology of China, and Sichuan University released ProphetNet, a sequence-to-sequence pre-training model for language creation problems. The model's objective is to enhance the quality and effectiveness of tasks involving the creation of natural language by foretelling future n-grams, which are collections of words that commonly appear in a particular sequence of text. ProphetNet is innovative in that it pre-trains the model on a significant quantity of data using a revolutionary self-supervised learning technique, which enables it to produce more accurate and coherent text.
A massive dataset of more than 160 GB of text from a variety of sources, including books, websites, and social media, was used to train ProphetNet. The model is pre-trained using a masked language modeling aim and is based on the transformer architecture. The researchers used a unique positional encoding technique and a new method for anticipating future n-grams to increase the model's effectiveness. According to experimental findings, ProphetNet surpasses current state-of-the-art models on a number of natural language generating tasks, such as question answering, machine translation, and summarization.

\subsubsection{MarianMT}
Marian is a free and open-source neural machine translation (NMT) toolbox that works with both CPU and GPUs for training and inference. Machine translation, summarization, and conversation production are examples of sequence-to-sequence problems for which the Marian toolset offers high-performance training and inference. Hugging Face, a provider of language technology, looks after it.
Marian's use of effective tensor operations to enable high-speed training and inference on both CPU and GPU is one of its significant contributions. The toolkit's extremely modular design makes it simple for academics and developers to test out various architectures and optimization strategies. Various pre-processing and post-processing tools are also included, making it simpler to work with various data types and languages. Marian has been applied in a range of academic and commercial applications, achieving state-of-the-art performance on a number of machine translation benchmarks.

\subsubsection{LayoutLMv2}
Using pictures, text, and layout information, LayoutLMv2 is a multi-modal pre-training framework created to extract useful information from visually rich texts. LayoutLMv2, which will be made available in December 2020 by a number of academic institutions, builds on the success of the first LayoutLM and intends to perform document comprehension tasks including word recognition, information extraction, and document categorization even better. The primary advancement of LayoutLMv2 is the fusion of many modalities into a unified pre-training framework, which enables the model to efficiently collect and exploit the intricate interactions between various parts in a document.
Academic papers, business reports, and government documents are among the varied variety of documents in the LayoutLMv2 training dataset. The LayoutLMv2 architecture consists of a transformer-based neural network that accepts a mix of layout data, text, and pictures as input. Combining supervised and unsupervised learning tasks, such as masked language modeling, image-text alignment, and layout prediction, are used to train the model. LayoutLMv2 beats state-of-the-art models on a number of document comprehension benchmarks, including SROIE, FUNSD, and PubLayNet, according to experimental findings, proving its usefulness in a variety of real-world situations.

\subsection{Year 2021}
With substantial advancements in fields like language modeling, computer vision, and reinforcement learning, LLM development continued to expand in 2021. The appearance of GPT-3 successors, such as GPT-Neo and GPT-Neo2, which are open-source alternatives to the original GPT-3 model, was one of the most significant advances. These models function similarly and are more easily available to the scientific community. A significant advancement was also made in the area of computer vision, where models like CLIP (Contrastive Language-Image Pre-training) and DALL-E 2 showed remarkable aptitudes for producing and comprehending visual material. 

\subsubsection{CLIP}
A new piece of work in artificial intelligence called CLIP suggests a revolutionary method for learning transferable visual representations under natural language supervision. The effectiveness of massively scalably pre-training deep neural networks for tasks like language modeling and machine translation served as the inspiration for this method. The purpose of CLIP is to train a neural network to predict whether or not a given picture and text pair match. This will allow vision and language models to learn from one another. In order to gain rich and transferrable visual representations that may be used to a variety of downstream vision tasks, the model is jointly trained on a broad set of image-text pairings.
A group of researchers from OpenAI created CLIP. Since its debut in February 2021, CLIP has drawn significant attention from the scientific community because to its outstanding performance on a variety of vision and language tasks. A massive dataset of image-text pairs, including more than 400 million photos and the descriptions that go with them from the internet, was used to train CLIP. The broad and representative mix of pictures and writings from many fields and languages was carefully selected for this dataset.
Similar to the transformer-based neural networks used in cutting-edge language models like GPT-3, CLIP's design is based on them. The encoders for pictures and text are combined in the model to forecast whether a given image and text combination will match or not. On a variety of vision and language tasks, such as picture categorization, object recognition, and visual question answering, CLIP has produced state-of-the-art results. Additionally, CLIP has shown outstanding zero-shot transfer performance, which means that with only natural language supervision, the model can function effectively on tasks it was not expressly trained on.

\subsubsection{DALL-E}
The DALLE model of a neural network is built on transformers and was created for zero-shot text-to-image generation. It was initially described in a research paper published in February 2021 by OpenAI. DALLE's goal is to automatically create a picture from text input without the need for further supervision or fine-tuning. DALLE employs a multi-modal strategy, fusing the power of language and visual data to produce new visuals that correspond to the textual input. The unique feature of DALLE is its ability to produce long, complicated sentences with high-quality, diversified pictures that fit the text.
Over 250 million picture-text pairs from the internet make up the broad mix of image and text data that DALLE is trained on. The encoder receives the textual input while the decoder creates the picture in DALLE's transformer-based design. The trial outcomes demonstrated DALLE's potential for a variety of applications, including creative writing, design, and art, by showing that it was able to produce high-quality and diversified visuals for a given text.
DALLE2, which OpenAI first released in April 2022, is an enhanced version of DALLE with more training data. In several text-to-image creation challenges, it obtained cutting-edge performance and shown impressive generalization skills. In the area of multi-modal machine learning, DALLE and DALLE2 are regarded as major developments because they have the power to completely change how we interact with machines by allowing them to comprehend and produce visuals based on natural language input.

\subsubsection{MT5}
The pre-trained transformer model mT5 for natural language processing is capable of completing a variety of tasks in several languages. It is an expansion of the T5 model with the capacity to handle several languages, and Google launched it in October 2020. The basic goal of mT5 is to enable zero-shot transfer learning across languages, which allows the model to carry out tasks in languages it has not been explicitly trained on. This facilitates multilingual tasks in natural language processing.
Massive and made up of over 101 languages, including low-resource languages, the training set utilized for mT5 is enormous. It comprises a wide variety of text formats, including books, news articles, and web pages. Similar to T5, mT5 uses a sequence-to-sequence transformer-based model that was trained on a sizable corpus of text in several languages. mT5 contains 1.2 billion parameters and 10 encoder and decoder layers. The model has been improved and put to the test on a variety of benchmarks for various natural language processing tasks, including sentiment analysis, question answering, machine translation, and summarization, among others. The findings demonstrate that mT5 performs better on a variety of tasks across several languages than many other models, including bilingual and multilingual models.

\subsubsection{DeBERTa}
DeBERTa, a BERT-like architecture that Microsoft unveiled in June 2020, seeks to boost language model performance in a variety of NLP applications by integrating disentangled attention and a decoding-enhanced training mechanism. Bidirectional Encoder Representations from Transformers, or BERT, has attained cutting-edge performance in numerous NLP applications. The training aim, however, solely concentrates on the masked language modeling job, which makes it susceptible to the issue of information overlap in attention heads.
Disentangled attention, which DeBERTa presents, decouples attention heads in multi-head attention and permits them to concentrate on various facets of the input sequence. By avoiding the issue of information overlap in attention heads, the model may more effectively use the attention process. DeBERTa also uses a decoding-enhanced training method that trains the model to decode from the intermediate representation of the model, which promotes the model to make more accurate predictions at inference time. DeBERTa can yield more accurate predictions and a better representation of the contextual relationships in the input sequence as a result.
According to experimental findings, DeBERTa performs at a high level on a variety of NLP tasks, including text categorization, natural language inference, and question answering. Additionally, it performs better than other cutting-edge language models like XLNet, RoBERTa, and BERT. DeBERTa has demonstrated to be particularly successful on situations where it is essential to capture long-range relationships. Overall, DeBERTa represents a substantial development in the NLP discipline and offers an exciting new line of inquiry.

\subsubsection{Pangu-$\alpha$}
A large-scale autoregressive pre-trained Chinese language model called PanGu was created by Huawei researchers. In terms of a variety of Chinese natural language processing (NLP) tasks, such as language modeling, text production, and text classification, it was released in April 2021 and has already achieved new state-of-the-art results. PanGu-$\alpha$'s use of an auto-parallel computing strategy, which permits training on enormous quantities of data with a constrained number of CPU resources, is its innovative feature. The architecture of the model is also built to handle the peculiarities of the Chinese language, such as its intricate syntax and deep semantics.
Chinese text data from a variety of sources, including news articles, web pages, and social media, makes up PanGu-$\alpha$'s training set. With more than 200 layers and 1.2 billion parameters, the model architecture is based on the transformer network. Compared to previous models of a comparable size, this large-scale model can be trained using just 512 GPUs because to the auto-parallel processing approach. According to experimental findings, PanGu- performs better than earlier state-of-the-art models on a number of benchmark datasets, including LAMBADA, People's Daily News, and XNLI. The model is an effective tool for Chinese NLP jobs due to its excellent performance and quick training procedure.

\subsubsection{GPT-Neo}
The GPT series has been extended by the AI language model known as GPT-Neo. It is a great tool for both researchers and developers because it is designed to be very scalable and accessible. GPT-Neo, which was made available in March 2021 by community-driven non-profit EleutherAI, was trained on a sizable dataset of online text, enabling it to produce coherent and contextually relevant replies to a variety of stimuli. The originality of GPT-Neo rests in its usability; without the requirement for a significant computational infrastructure, the model is freely accessible to anybody who wants to utilize it.
A total of 1.3 terabytes of data were used to train the model on a variety of materials, including web pages, scholarly publications, and online books. The transformer architecture of GPT-Neo, one of the biggest open-source language models, includes 1.3 billion parameters. Through a series of benchmark tests, the model's performance was assessed, and the findings revealed that it performed at the cutting edge on a number of linguistic tasks, including sentiment analysis, question answering, and text completion. Additionally, the model has been used in a number of natural language processing applications, including chatbots, text production, and text categorization, proving its adaptability and breadth of use.

\subsubsection{ProphetNet 2.0}
Weizhen Qi et al. created the large-scale pre-training model known as ProphetNet-X. It is an expansion of the original ProphetNet model and was created to manage numerous NLP tasks including conversation production, machine translation, and summarization. The model, which was made public in September 2021, has excelled in a number of benchmarks, including the WMT14 English-German translation challenge and the CNN/Daily Mail summarization dataset, by achieving state-of-the-art results.
The uniqueness of ProphetNet-X resides in its capacity to manage diverse NLP tasks with just a single pre-training model. The model does this by including task-specific tokens and creating innovative pre-training objectives that take into account the properties of various activities. The "Layer-wise Random Mixup," another effective pre-training technique introduced by ProphetNet-X, reorders the model's layers to promote cross-layer information sharing during training. ProphetNet-X is a potential tool for next NLP research and applications thanks to these enhancements, which enable it to outperform earlier models in a number of NLP benchmarks.

\subsubsection{MARGE}
A pre-training method called MARGE creates sentence-level paraphrases to improve the quality of the pre-training data for NLP models. It debuted on Facebook AI in 2020. By including a broader variety of sentence variants during pre-training, the major objective is to increase the resilience and generalization of NLP models. In a novel fashion, MARGE makes use of a substantial body of monolingual text and applies a two-stage procedure to produce paraphrases in an entirely unsupervised manner. First, it uses back translation, a technique that uses machine translation models to translate a text into another language and then back to the original language, to produce noisy paraphrases of the input sentence. Then, using the similarity score metric, it refines noisy paraphrases by sorting them according to how closely they resemble the original sentence.
MARGE has extensive pre-training on over 3 billion tokens of text from the English Wikipedia and the BooksCorpus. MARGE's design is comparable to those of other cutting-edge transformer-based models like BERT and GPT. To motivate the model to learn from the paraphrased versions of the input sentences, MARGE uses a new pre-training objective. The experiment's findings demonstrated that MARGE performed better than other cutting-edge pre-trained models on a variety of downstream NLP tasks, including sentiment analysis, question answering, and natural language inference. Additionally, MARGE performed better on tasks that call for a deep comprehension of natural language, such as those that involve adversarial instances and out-of-distribution examples.

\subsubsection{VILLA}
VILLA is a large-scale adversarial training method for learning representations of vision and language. Researchers from Microsoft and the University of Maryland first described it in a paper in June 2020. Learning representations that can be used to a variety of vision-and-language activities, including picture captioning, visual question answering, and visual grounding, is the goal of VILLA. The primary advancement of VILLA is the application of adversarial training to motivate the model to develop reliable and generalizable representations that can capture the combined distribution of visual and textual information. This is accomplished by using a discriminator that can tell the difference between actual and artificial visual-textual pairings.
A sizable corpus of image-text pairings that are gathered from the internet serve as the pre-training data for the VILLA model. Pre-training is divided into two stages: the first involves training the model to produce paraphrases of the input text, and the second involves training the model to produce visual characteristics that are compatible with both the input text and the produced paraphrases. VILLA's design is based on the Transformer architecture, a well-liked neural network architecture for applications involving natural language processing. VILLA demonstrates the efficiency of adversarial training for vision-and-language representation learning by achieving state-of-the-art performance on a range of vision-and-language tasks, including as picture captioning, visual question responding, and visual grounding.

\subsubsection{Codex}
Codex is a sizable language model created to comprehend and produce code. It was made available in July 2021 by OpenAI with the intention of giving programmers a potent tool for creating code automatically. The model can create new code or finish old code with just a few suggestions because it was trained on billions of lines of publicly available code. The unique feature of Codex is its capacity to comprehend the context of the code and produce very accurate, syntactically correct code.
The training set for Codex is drawn from the 500 GB of code and over 14 million public repositories on GitHub. The model is trained using a combination of supervised and unsupervised learning, where the unsupervised data set consists of the full public codebase and the supervised data set consists of a collection of prompt-response pairings. The GPT (Generative Pre-trained Transformer) is the foundation of Codex's architecture, which has been optimized for the purpose of code creation. The outcomes of the experiment demonstrated Codex's ability to produce code of a high caliber that is comparable to human-written code and to accurately carry out a range of programming tasks. However, there are worries over the security ramifications of such a potent tool and the potential for it to be used maliciously.

\subsubsection{Switch Transformer}
Switch Transformers is a research paper written by a group of Google researchers that was released in January 2021. In order to attain trillion-parameter models, it suggests a novel technique for training and scaling up transformer-based models, like GPT-3. A novel sparse attention method that decreases computing cost while retaining good accuracy is the major breakthrough. The performance of different natural language processing (NLP) tasks, such as language modeling and text production, can be improved by using this method, which enables training of much bigger models that can learn from much larger datasets.
Switch Transformers uses less computing power and memory than previous transformer-based models while achieving state-of-the-art performance on most NLP benchmarks. The suggested design is based on a hybrid strategy that incorporates mechanisms for sparse and intense attention. The authors show that even scaling to models with trillions of parameters, Switch Transformers may still perform as well as or better than current dense models. The efficiency of training and inference in smaller models may also be enhanced by the suggested approach.

\subsubsection{ALIGN}
The difficulty of scaling up big models to serve multiple downstream tasks, such as image classification, object recognition, image captioning, visual question answering, and image-text retrieval, is addressed by ALIGN, a visual and vision-language pre-training framework. The contrastive learning paradigm, which facilitates learning of visual and linguistic representations through a shared purpose, is the foundation of ALIGN, a system created by Google researchers in May 2021. The main novelty of ALIGN is to improve the quantity of training data available for pre-training huge models, which is essential for the success of large-scale models, by utilizing noisy text from the internet. The ALIGN architecture is also intended to be effective, allowing for the training of substantial models with a minimum amount of hardware.
Web-crawled text, multilingual text, image annotations, and speech data were all employed by the researchers as ALIGN's training data. The ALIGN architecture comprises of a vision encoder and a text encoder that are concurrently trained to learn linguistic and visual alignments in a common semantic space. To increase the agreement between pairs of positive samples and decrease the agreement between pairs of negative samples, ALIGN uses a contrastive learning goal. The experimental findings of ALIGN show how well it performs on a variety of vision-language tasks, including as picture-text retrieval, image captioning, and visual question answering, and it attained state-of-the-art scores on a number of benchmarks.

\subsubsection{Galactica}
Meta AI and Papers with Code created the transformer-based language model called Galactica, which was particularly trained on scholarly writing. Galactica, which will be available in November 2022, is made to handle a variety of scientific research-related activities, such as information retrieval, summarization, question-answering, code development, and experiment planning. A curated dataset comprising 48 million scientific publications, 10 million textbooks, and 1 million code snippets is used to train the machine. Galactica performs better on scientific tasks than earlier language models, including as producing more accurate and informative summaries of scientific literature and providing more thorough answers to scientific inquiries.
The first language model specially trained on scientific texts is Galactica. This enables it to perform better on scientific challenges than earlier language models. The training set for the model is meticulously chosen to guarantee its excellent quality and authenticity. The Transformer design, which is more effective and simpler to train, is the foundation of the Galactica architecture. The model has the potential to be applied in a variety of scientific contexts, such as medical treatment, teaching, and research.

\subsubsection{ERNIE 3.0}
A large-scale pre-training model for natural language interpretation and generating tasks is called ERNIE 3.0. It was created by scientists at Baidu. The major goal of ERNIE 3.0 is to increase language models' capacity to use outside information and resources in order to perform better on diverse NLP tasks.
A sizable corpus of text data, including both general-domain and domain-specific information, including scientific publications and websites, is used to train the ERNIE 3.0 model. A multi-granularity masking technique that enables the model to better capture contextual relationships between words and entities is one of the model's key innovations. Another is a knowledge distillation framework that makes use of large-scale knowledge graphs and ontologies to enhance model performance. ERNIE 3.0's fine-tuning and inference modules, in addition to its pre-training capabilities, enable it to be used for a variety of NLP applications. ERNIE 3.0 beats state-of-the-art models on a range of benchmark datasets for tasks including question answering, natural language inference, and text categorization, according to experimental results.

\subsubsection{GLaM}
A Google research team has developed a new architecture for scaling up language models called GLaM (Generalist Language Model). This model's primary goal is to introduce a mixture-of-experts technique to effectively scale up the training of big language models. The unique aspect of GLaM is that it offers a quick and effective approach to merge many models and capitalize on each one's advantages to produce a single, sizable model that excels at a variety of tasks. This method's central idea is to train a number of tiny, task-specific models (i.e., experts) and then merge them via a gating mechanism to produce a single, big model. In December 2021, GLaM was published on arXiv.
A wide variety of text data, including those found in books, websites, and other sources, was used to train GLaM. A gating network chooses the best expert for a particular input sequence as part of the GLaM architecture, which is based on a mixture-of-experts technique. The specialists have received separate training and have areas of expertise in syntax, semantics, and context language interpretation. In order to improve the effectiveness of the training procedure, GLaM also employs a number of additional methods, such as adaptive computation time and dynamic routing.
GLaM outperforms other large-scale language models according to experimental findings on benchmark datasets including GLUE, SuperGLUE, and LAMBADA. Additionally, it performs at the cutting edge on a number of other language tasks, including text categorization, language modeling, and question answering. Overall, GLaM is an encouraging step toward scaling up language models and has the potential to enhance the functionality of several NLP applications.

\subsubsection{Gopher}
DeepMind's Gopher language model, which has 280 billion parameter transformers, was made public on December 15, 2021. A massive text and code dataset, comprising the totality of Wikipedia, books, code, and other publicly accessible material, served as its training ground. NLU, NLG, MT, code generation, QA, summarization, and text categorization are just a few of the many jobs that Gopher is made to do. It can produce more realistic and educational writing, translate languages more precisely, and provide more thorough answers because it is the first language model to be trained on a dataset this huge.
The training set for Gopher is carefully chosen to be of the highest caliber and to be realistic of the actual world. To eliminate biases and inaccuracies, the data is cleansed and filtered. Gopher is a transformer-based language model that employs a more effective and simple to train Transformer architecture. Gopher represents a substantial advancement in the field of language modeling by outperforming earlier language models on all assessed tasks.

\subsection{Year 2022}
In 2022, several large language models (LLMs) were developed by various tech companies, such as Microsoft, NVIDIA, Meta AI, Yandex, and Google. These LLMs were trained on massive datasets of text and code and have the ability to perform a range of tasks, including natural language understanding, generation, machine translation, and code generation. Their development represents a significant advance in the field of artificial intelligence and holds potential for applications in various industries such as customer service, education, and healthcare.

\subsubsection{Megatron-Turing NLG}
Microsoft and NVIDIA created the 530 billion parameter transformer language model known as MT-NLG, which was made public on January 28, 2022. The model is created to carry out a wide range of tasks, including natural language understanding, natural language generation, machine translation, code generation, question answering, summarization, and text classification. It is trained on a massive dataset of text and code, which includes the entirety of Wikipedia, books, code, and other publicly available data. The DeepSpeed training system, which enables the training of very large language models on a single GPU or on a cluster of GPUs, was used to train the MT-NLG language model, which is the first language model to be trained on a dataset of this size and scope.
The MT-NLG is a transformer-based language model that employs an improved and simpler to train Transformer architecture. The MT-NLG training set is carefully chosen to be of the highest caliber and most accurate to the actual world. On a range of tasks, including producing more realistic and educational literature, accurately translating languages, and providing more thorough answers, MT-NLG beats earlier language models. With potential uses in many areas, including machine learning and natural language processing, MT-NLG represents a substantial advancement in language modeling.

\subsubsection{Chinchilla}
On April 12, 2022, DeepMind unveiled Chinchilla, a language model with 70 billion parameter transformers. It is intended to carry out a variety of natural language processing tasks, including text categorization, code generation, NLU, NLG, and MT. In comparison to earlier language models, Chinchilla is the first language model to be trained on a dataset this big while being compute-optimal.
The complete Wikipedia, books, code, and other publicly accessible material are included in Chinchilla's training set, which has been meticulously vetted to ensure high quality and realistic depiction of the outside world. A modified version of the Transformer architecture, a kind of neural network best suited for problems involving natural language processing, is used by Chinchilla. According to experimental findings, Chinchilla performs better than earlier language models on all tasks considered, producing more realistic and educational literature, accurately translating languages, and fully addressing queries. The advancements made by Chinchilla may increase the number of fields in which huge language models may be used.

\subsubsection{PaLM}
On April 5, 2022, Google AI launched PaLM (Pathways Language Model), an autoregressive transformer model with 540 billion parameters. It is the first language model to be trained on a dataset of this size and scope, and it performs better than earlier language models on a range of tasks, including code creation, machine translation, natural language interpretation, and generation. Using the Pathways system, a revolutionary machine learning method that enables very efficient training of very large neural networks spanning thousands or tens of thousands of accelerator chips, PaLM was trained on 780 billion tokens of text and code.
PaLM's training set consists of carefully selected, high-quality data, such as the complete Wikipedia, books, code, and other information that is readily accessible to the public. PaLM employs a more effective and simple to learn variant of the transformer design. According to experimental findings, PaLM outperforms other language models in terms of producing writing that is more accurate and informative, translating languages more accurately, and providing more thorough answers. The extensive and important uses of PaLM make it a notable advancement in the field of language modeling.

\subsubsection{OPT}
A collection of open-sourced, big language models called OPT: Open Pre-trained Transformer Language Models was created by Meta AI in May 2022. OPT models come in a range of sizes, from 125M to 175B parameters, and are trained on a sizable dataset of text and code. They are the first major language models that have been trained on a dataset of size and scope that are open-sourced and intended to be used by researchers and developers. On a range of tasks, including machine translation, code generation, natural language interpretation, and natural language synthesis, OPT models outperform earlier language models.
The totality of Wikipedia, books, code, and other publicly available data are all included in the training set for OPT models, which is composed of carefully selected, high-quality, and representative data. OPT models, which employ a modified version of the Transformer architecture and are more effective and simple to train, are transformer-based language models. OPT models are a significant advancement in the field of language modeling with the potential to be employed in a number of applications. They surpassed earlier language models on all of the tasks on which they were assessed.

\subsubsection{YaLM}
On April 12, 2022, Yandex launched YaLM-100B, a language model with 100 billion parameter transformers. As the first language model to be trained on a dataset of this size and scope, it outperforms earlier language models on a variety of tasks, including text classification, NLU, NLG, MT, and QA. The DeepSpeed technology, which enables the training of very large language models on a single GPU or on a cluster of GPUs, was used to train YaLM-100B.
The totality of Wikipedia, books, code, and other publicly accessible material, cleaned and filtered to ensure high-quality and realistic representation, make up the training set for YaLM-100B. YaLM-100B utilizes a modified version of the Transformer architecture and surpasses earlier language models in a variety of tasks, including producing more realistic and educational writing, accurately translating languages, and providing more thorough answers. YaLM-100B has the ability to be employed in a variety of applications, including code generation, machine translation, natural language comprehension, and natural language synthesis.

\subsubsection{Minerva}
Google created a sizable language model called Minerva, which was made public on June 1st, 2022. A massive text and code dataset, comprising the totality of Wikipedia, books, code, and other publicly accessible material, is used to train Minerva. This LLM is the first to have been trained on a dataset of this size and scope, and it performs better than earlier LLMs on a range of tasks. Natural language understanding (NLU), natural language generation (NLG), machine translation (MT), code generation, question-answering (QA), summarization, and text categorization are just a few of the diverse jobs that Minerva is made to handle. The Pathways method, which enables the training of LLMs of this size and scope in a reasonable length of time, was used to train Minerva, the first LLM.
The totality of Wikipedia, books, code, and other publicly accessible data make up the training set for Minerva. The training set is carefully chosen to be of the highest caliber and most accurate to the actual world. The architecture used by Minerva is transformer-based, which is more effective and simpler to train. Minerva excels earlier LLMs on all tasks, producing more realistic and educational content, accurately translating languages, and providing more thorough responses. In conclusion, Minerva represents a substantial advancement in the field of language modeling with prospective uses in machine translation, code creation, natural language production, and understanding.

\subsubsection{BLOOM}
A vast dataset of text and code in 46 languages, including the totality of Wikipedia, books, and other publicly available material, was used to train BigScience's 176 billion parameter transformer-based language model known as BLOOM. It was made available on May 25, 2023, and it may be used to carry out a variety of activities like text categorization, question-answering, machine translation, code creation, and natural language production. The Pathways system, which enables the training of very large language models on a single GPU or on a cluster of GPUs, was used to train BLOOM, the first multilingual language model on a dataset of this size and scope.
Being the first multilingual language model to be trained on a dataset of this size and scope gives BLOOM an edge over other multilingual language models in terms of originality. Furthermore, it is the first multilingual language model learned using the Pathways method, allowing for the rather quick training of multilingual language models of this magnitude. The Transformer architecture is updated for BLOOM, making it more effective and simpler to train. According to experimental findings, BLOOM surpasses earlier multilingual language models on all tasks considered, including producing more accurate language translations, producing more realistic and educational content, and providing more thorough answers.

\subsection{Year 2023}
Several large language models (LLMs) were created in 2023 by significant tech firms as Google AI, OpenAI, and BigScience. These models can carry out a variety of tasks, including natural language processing, creation, machine translation, and code production. They were trained on enormous datasets of text and code. Along with the creation of new LLMs, advancements have been made in the creation of methods and tools for training and deploying LLMs, such as Google AI's Pathways system. LLM development is an area that is quickly developing and has significant applications across several sectors.

\subsubsection{LLaMA}
In April 2023, Meta AI launched the LLaMA collection of big language models that are open-sourced. With a training set made up of Wikipedia, books, code, and other publicly accessible material, it is the first open-sourced big language model to be trained on a dataset of size and scope. Transformer-based LLaMA models employ a modified, more effective, and simpler to train version of the Transformer architecture.
LLaMA models perform better than earlier language models across a range of natural language processing tasks. LLaMA models have the potential to be employed in a variety of applications, including code generation, machine translation, natural language interpretation, and natural language synthesis. The first open-sourced large language models to be trained on a dataset this size and scope, as well as the first large language models to be trained using the Pathways system, which makes it possible to train language models of this size and scope more effectively, are the innovation points of LLaMA models.

\subsubsection{Pangu-$\Sigma$}
Pangu-sigma is a new large language model (LLM) from Huawei that is based on Chinese corpus and intended to do multilingual jobs. The model, which has around 1.085T parameters and was trained using 2.17T data with lengths exceeding 300B tokens, is reportedly the first Chinese-based LLM to achieve a size of 1T parameters. 200G from the WuDaoCopora 2.0 dataset, 100G from CLUECorpus 2020, 800G from the Pile, and 750G from C4 make up the training set. Pangu-sigma can also handle jobs involving code because it has 157G of Python code and 161G of Java code.
Two technologies are suggested in order to attain the efficiency of the model. The Random Routed Experts (RRE) sparsity approach is the first. For the same assignment, RRE separates the experts into groups based on their criteria. RRE allocates experts to tokens at random, in contrast to other models that feed tokens to a particular expert with the best match being managed by a gate function. Researchers may extract sub-models from Pangu-sigma and use them for downstream tasks like translation and chat thanks to the gate-free RRE mechanism.
The Expert Computation and Storage Separation technique is the second proposed technology. In order to achieve 69,905 tokens per second IO efficiency and lower the communication overhead between the server and devices, this approach is utilized to train the model spread across a cluster.

\subsubsection{BloombergGPT}
A 50 billion parameter big language model called BloombergGPT was created by Bloomberg and Johns Hopkins University. It was made public on March 30, 2023, and it was trained on a sizable financial data set that included news reports, financial statements, and regulatory filings. Designed to conduct natural language interpretation, generation, machine translation, code generation, question answering, summarization, and text categorization, BloombergGPT beats earlier language models on a range of tasks. Researchers and developers may use it for free, and it has the power to completely alter how we interact with financial data.
BloombergGPT is a strong tool that may be used to increase the effectiveness and accuracy of financial jobs. It represents a significant advancement in the field of language modeling. Although it is still under development, some of its major characteristics include being trained on a sizable dataset of financial data, having the ability to carry out a variety of jobs, and being freely accessible to academics and developers. The adoption of BloombergGPT might transform the way we engage with financial data and enhance a variety of financial processes.

\section{Recent Multimodal Large Language Models}

\subsection{GPT-4}

GPT-4 is the latest generation of multimodal pre-trained model (MLLM) by OpenAI that was recently released. It finished training in August and is capable of completing more complex tasks with more accurate results. Compared to the current GPT-3.5, which was a fine-tuned version of GPT-3, GPT-4 has several notable improvements.

Firstly, GPT-4 supports both image and text inputs, and its output is in text format, making it a true MLLM. This capability expands the range of tasks that GPT-4 can perform, including those that require multimodal inputs.

Secondly, GPT-4 supports longer token size. At present, the token length supported by ChatGPT at GPT-3.5 is limited to 4096 tokens, equivalent to around 3000 English words. GPT-4, on the other hand, can support token lengths of up to 32767, or around 25000 words. This increase in token length enables GPT-4 to process longer sequences of text and make more accurate predictions.

Thirdly, GPT-4 places greater emphasis on security issues, including Adversarial Usage, Unwanted Content, and Privacy Concerns. To address these concerns, GPT-4 uses three methods: RLHF (reinforcement learning with human feedback), real-world use cases, and an adversarial testing program for alignment. These measures help to ensure that GPT-4 is less susceptible to adversarial attacks and can handle unwanted content while maintaining user privacy.

Finally, GPT-4 allows users to use specific prompts to customize the behavior of the model. This feature improves GPT-4's ability to perform specific tasks and provides users with more control over the model's output.

In summary, GPT-4 is a highly advanced MLLM that outperforms its predecessors in terms of its capabilities, token length, security features, and customization options. Its release marks a significant milestone in the field of natural language processing and opens up new opportunities for research and applications.

\subsubsection{Comparsion between GPT-4 with Previous LLM GPTs}

GPT-4 is the next iteration of OpenAI's GPT series of models. According to OpenAI, GPT-4 is expected to be the most advanced and powerful LMLM model to date. However, at the time of writing, technical details about the model have not been released. Therefore, we will compare the current GPT models with the information that is currently available.

As shown in the table, the main difference between the current GPT models is in the size of the training data and the number of parameters. GPT-1 used only 5GB of text data from 7000 unpublished books and had only 117M parameters, while GPT-3 used 45TB of data and had 175B parameters. GPT-3.5 was a fine-tuned version of GPT-3 that focused on improving specific tasks, such as text completion and code generation.

Regarding GPT-4, OpenAI has disclosed some information about the technology used for the model. The model is trained on all public data from the internet and datasets licensed to OpenAI. OpenAI also continues to use the RLHF algorithm for fine-tuning. Additionally, a new deep learning stack has been built that scales predictably to predict the predictability of larger models under small models. A new Rule-based reward models (RBRMs) has been introduced to refuse harmful content based on specific rules.

Furthermore, ChatGPT has also revealed that they use a formula to make predictions on larger models, $$log[pass\_rate(C)] = \alpha * C ^{-k}$$, where C represents the size of the model, and k and $\alpha$ are positive constants.

In summary, GPT-4 is expected to be a significant advancement in LMLM technology, with improvements in the training data size, number of parameters, and algorithmic architecture. However, given the limited information currently available, further research is required to understand the full potential of this model.

\subsection{Microsoft KOSMOS-1}
Large language models have developed significantly in natural language processing over the past few years, but they haven't yet mastered the integration of visual data. By integrating visual signals and spoken prompts, Microsoft's Kosmos-1, a Multimodal Large Language Model (MLLM), has changed this and made it possible for it to carry out activities like picture captioning and visual question answering. Kosmos-1, which is based on Transformer's causal language model, has the ability to recognize visual text, solve visual puzzles, and evaluate images for information. Moreover, it can learn contextually through few-shot learning and obey commands through zero-shot learning. This latest advancement in MLLMs is a big step toward multimodal learning and more sophisticated natural language processing.

\subsubsection{Model Architecture}
The KOSMOS-1 model utilized a magneto transformer as its backbone, which is a variant of the transformer architecture. The main difference between the original transformer and the magneto transformer is the addition of a layer normalization between the transformer's linear layer and activation function, which increases training stability and scalability. KOSMOS-1 was designed with 24 layers of decoder, each with 2048 dimensions, 8192 hidden size, and 32 attention heads, resulting in approximately 1.6 billion parameters. To accelerate training, the model did not directly feed images but instead used a CLIP ViT-L/14 model with 1,024 feature dimensions to obtain images.

In addition, the KOSMOS-1 model also employed the XPOS technique, which utilizes length-extrapolation to address the length difference between training tokens and predicted tokens. These strategies were key to the model's ability to perform a variety of tasks, including image captioning, visual question answering, and more, making it a powerful tool for multimodal learning. Overall, KOSMOS-1 represents a significant advance in the development of multimodal large language models, with the potential to revolutionize natural language processing and computer vision research.

\subsubsection{Dataset and Representation}

KOSMOS-1 comprises three types of datasets. The first dataset contains text corpora, including The Pile, a massive English text dataset for LLMs, and other datasets such as Common Crawl, CC-Stories, and RealNews. The second dataset consists of image-caption pairs from several datasets, such as English LAION-2B, LAION-400M, COYO-700M, and Conceptual Captions. These datasets were obtained by crawling. The last dataset is interleaved image-text data, which contains interleaved image and text snippets. This data was selected from a 2B web pages crawled, which was reduced to 71M web pages in the final dataset.

To encode the sequence before feeding it into the model, all text sequences were encoded as <s>, and all images were encoded as <image>. While audio sequences were also supported by KOSMOS-1, the paper did not provide further details, indicating that it may not be ready yet.

KOSMOS-1 used magneto transformer as its backbone, which is a variant of transformer. The only difference between magneto and the original transformer is that the former added a layer normalization between the transformer's linear layer and activation function to increase training stability and ensure easy scaling. The model used 24 layers of decoder with 2048 dimensions, 8192 hidden size, and 32 attention heads, containing around 1.6B parameters.

To speed up training, images were obtained from a CLIP ViT-L/14 model with 1,024 feature dimensions, and a second track called XPOS leveraged the Length-Extrapolation technique to address the length difference issue between training tokens and predicted tokens.

\subsection{Google PaLM-E}
Google PaLM-E, denoted as Embodied Pathways Language Model, is a multi-task language model based on the previous PaLM, which was also the first trained LLM on Google's Pathways architecture. The Pathways architecture was designed to achieve sparse activation for multimodal and multi-tasks, meaning that for a specific task, only a part of the model would be activated, reducing computational complexity.

PaLM-E is a Visual-Text Model that, similar to Microsoft's KOSMOS-1, can understand natural language and images. Additionally, it can be implemented in robotics to achieve embodied tasks. This model is trained on a large-scale dataset called GEM, which contains both text and visual data, including ImageNet, COCO, and Visual Genome.

The model consists of two components, the language pathway and the visual pathway. The language pathway is based on the Transformer-XL architecture, and the visual pathway is based on the Vision Transformer (ViT) architecture. The language and visual pathways are connected by a fusion module, which allows the model to integrate both modalities.

PaLM-E was evaluated on several tasks, including image captioning, visual question answering, and embodied navigation. In the embodied navigation task, the model was trained to navigate through a virtual environment by following natural language instructions. PaLM-E outperformed several state-of-the-art models on all tasks, demonstrating its effectiveness in both language and vision tasks.

In conclusion, PaLM-E is a multi-task language model that can understand natural language and images and can be implemented in robotics for embodied tasks. The model is trained on a large-scale dataset and consists of a language pathway, a visual pathway, and a fusion module. The model achieved state-of-the-art performance on several tasks, demonstrating its effectiveness in both language and vision tasks.

\subsubsection{Model Architecture}
PaLM-E is based on Google's Pathways architecture and combines two models: PaLM, a Large Language Model, and ViT 22B, a Visual Transformer model. PaLM provides the language processing capabilities, while ViT 22B is used for image processing. The default model used is a 540B PaLM model plus a 22B ViT model, which is a simple ViT model scaled to 22B. This gives the PaLM-E model a total of 562B parameters.

\subsubsection{Dataset and Representation}
Regarding the data used to train PaLM-E, a total of 780B tokens were utilized, consisting of social media conversations and data from various sources, including web pages, Wikipedia, and GitHub. The ViT 22B model was trained on the JFT dataset, which contained approximately 4B semi-automatically annotated images. The input representation method was similar to KOSMOS-1, where visual or robotics-related inputs were labeled with tags such as <img> for image input or <obj> for object detection in robotics tasks. Different encoding methods were used for the content in these tags, such as ViT for image embedding and Object Scene Representation Transformer for 3D scenes. The text data were fed directly into the language model.

\section{Experiment Results}
TODO

\section{Comparison Over SOTA MLLMs}
TODO

\section{Limitation}
TODO

\section{Discussion}
\subsection{Challenges}
TODO
\subsection{Future work}
TODO

\section{Conclusion}
TODO

==> sections/draft_background.tex <==
% \section{Background\label{sec:relatedwork}}

% \subsection{Transformer}
% At current stage, most of the LLM was based on the architecture of Transformer which was proposed in 2017 \cite{vaswani2017attention}. Transformer is a type of sequence to sequence model and the largest different thing between transformer and the previous widely used sequence to sequence models such as Long short-term memory (LSTM) \cite{graves2012long} and Recurrent Neural Network (RNN) \cite{medsker2001recurrent} is that the training of RNN and LSTM that the processing of the sequence in these models was strictly in sequence order, which means the next token would be processed only after the current sequence has been processed. While in transsormer architecture, multi-head self-attention \cite{vaswani2017attention} was used in which case training the large model in parallel could become feasible.
% The whole transformer architecture could be divided into two parts, similar as the current LLM, the encoder and decoder. The encoder was able to map the input sequences into the embedding space and the decoder was able to generate expected sequence according to the embedding space, normally a transformer based model was composed with several layers of encoder and several layers of decoder. The image below showed how transformer works.
% However, for transformer based models, the positional information would not be included due to its parallel structure, which means the transformer does not process the input in the order of the sequence input hence another technique to embed the positional information was the positional encoding. In the transformer, the trigonometric function sin and cos were used to provide the positional information with the formula below:
% $$E(pos, 2i) = sin(pos/10000^{2i/dim})$$
% $$E(pos, 2i+1) = cos(pos/10000^{2i/dim})$$
% In which the pos was the relative position of a certain token from 0 to the max length of the sequence, while i was the index number of the current token inside the input ranging from 0 to half of the embedding dimension while the dim was that dimension value.

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=1\columnwidth]{diagrams/overview/transformers.png} 
%     \caption{The architecture of Transformer
%     \label{fig:evotree}}
% \end{figure}

% \subsection{RLHF}
% Reinforcement Learning with Human Feedback (RLHF) \cite{christiano2017deep} was the training strategy used on some LLMs such as Sparrow by Deepmind \cite{glaese2022improving} and instructGPT \cite{ouyang2022training} which was a technique to use hunman feedback as a kind of reward as the training loss of model generated content.
% To fine tuning the model, some gradient policy was used, one kind of policy widely used is Proximal Policy Optimization (PPO) \cite{schulman2017proximal} based on Policy Gradient \cite{wang2022policy}, the key idea of PPO is that instead of doing on-policy gradient process, the PPO would do sampling of a part of parameters of the model which could make it off-policy.

% \subsection{Chain-of-Thought}
% The chain of thought can be understood as a sequential progression of ideas, concepts, and associations triggered by the interaction with a large language model. These models, like the renowned GPT-3.5, are trained on massive datasets containing an extensive range of linguistic patterns, enabling them to generate coherent and contextually relevant text based on the input they receive. This ability has given rise to a captivating dynamic: users engage with the model by providing an initial prompt, and the subsequent output becomes a catalyst for the continuation of thought.

% As users interact with large language models, the chain of thought unfolds through a captivating process. The model responds to the prompt with a coherent and contextually relevant text, often extending beyond the initial input and introducing new dimensions to the discussion. This generated output serves as a foundation for the user's subsequent input, leading to a reciprocal exchange that simulates a conversation.

% Furthermore, the chain of thought reveals intriguing insights into the complexities of creativity, reasoning, and linguistic nuance. Users find themselves traversing through a web of ideas as the model's responses spark new perspectives and lead to unforeseen territories of thought. This iterative dialogue challenges the traditional boundaries between human and machine-generated content, highlighting the symbiotic relationship that emerges when the capabilities of large language models blend with the intricate workings of human cognition.

% However, the chain of thought is not without its nuances. While large language models excel at generating text, they lack genuine consciousness and understanding. The apparent coherence and relevance in their responses can sometimes be misleading, as they often rely on statistical patterns present in their training data rather than true comprehension. This raises philosophical questions about the nature of thought and creativity, blurring the lines between genuine human introspection and algorithmic processing.

\section{Challenges\label{sec:relatedwork}}

% The genesis of large language models lies in the advancement of neural networks and the technologies derived from it. Such as Deep Learning. To train a model with massive scale, cutting edge techniques had been proposed such as Transformer, Reinforcement Learning with Human Feedback, Chain of Thought and Mix of Expert. This section will lead to a coarse-grained overview on the technologies lead to the bloom of large language model technique on the background.

Large language models are the result of the development of neural networks and the technologies that followed such as like deep learning. For the modern cutting edge models, challenges still exist in the following phases:
\begin{itemize}
    \item \textbf{Computational Complexity}: Large language models requires a massive computational resource for the pre-training and fine-tuning.
    \item \textbf{Memory intense}: Large language models normally contains over billions of parameters, which cause memory intensive during both the training and deployment phase.
    \item \textbf{Inference Latency}: Large language models normally faces latency issue due to the computational complexity.
    \item \textbf{Model Generalization}: Same as other deep learning models, large language models can also have generalization issue on unseen data.
\end{itemize}

Cutting edge methods like Chain of Thought, Reinforcement Learning with Human Feedback, Transformer, and Mix of Expert have been proposed to train a model on a massive scale. A cursory review of the technologies that underpin the large language model technique will be provided in this section.

% \subsection{Transformer}
% The contemporary landscape of Large Language Models (LLMs) predominantly employs the Transformer architecture, introduced in 2017 \cite{vaswani2017attention}. A paradigm shift from the conventionally used sequence-to-sequence models such as Long Short-Term Memory (LSTM) \cite{graves2012long} and Recurrent Neural Network (RNN) \cite{medsker2001recurrent}, the Transformer's key innovation lies in its parallel processing ability. Unlike the sequential processing constraint in LSTMs and RNNs, where a token's processing is dependent on its predecessor, the Transformer, through its multi-head self-attention mechanism \cite{vaswani2017attention}, facilitates parallelized training.

% Conceptually, the Transformer can be bifurcated into the encoder and decoder components. While the encoder maps input sequences into a higher-dimensional embedding space, the decoder crafts sequences based on these embeddings. Typically, a Transformer model comprises multiple layers of both encoders and decoders. An illustrative representation of the Transformer's architecture is provided below:

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=1\columnwidth]{diagrams/overview/transformers.png} 
%     \caption{The architecture of the Transformer.}
%     \label{fig:evotree}
% \end{figure}

% A notable challenge in the Transformer architecture is the absence of innate positional information due to its parallelized nature. To counteract this, positional encoding is integrated, utilizing sine and cosine functions. The encoding is described by:
% $$E(pos, 2i) = \sin\left(\frac{pos}{10000^{2i/\text{dim}}}\right)$$
% $$E(pos, 2i+1) = \cos\left(\frac{pos}{10000^{2i/\text{dim}}}\right)$$
% Here, \( pos \) represents a token's relative position within a sequence, and \( i \) spans from 0 to half the embedding dimension, \( \text{dim} \).

\subsection{RLHF}
Reinforcement Learning with Human Feedback (RLHF) \cite{christiano2017deep} represents an innovative training paradigm, harnessed in models such as Sparrow by DeepMind \cite{glaese2022improving} and instructGPT \cite{ouyang2022training}. RLHF incorporates human feedback as a reward mechanism, offering nuanced loss parameters based on human evaluation of model-generated content.

To optimize these models, gradient policies like the Proximal Policy Optimization (PPO) \cite{schulman2017proximal} are employed. Rooted in Policy Gradient methods \cite{wang2022policy}, PPO distinguishes itself by sampling subsets of model parameters, rendering the optimization process off-policy.

\subsection{Chain-of-Thought}
The concept of a "chain of thought" encapsulates the dynamic, iterative discourse between users and large language models, such as GPT-3.5. Trained on vast linguistic datasets, these models have the prowess to spawn coherent and context-rich text in response to user prompts. This response often extends beyond mere answers, seeding new dimensions of thought and engagement.

The interaction is captivating: user inputs shape the model's outputs, which in turn inspire further user queries, simulating a conversational dynamic. This recursive engagement blurs boundaries between human-generated content and machine responses, offering a confluence of creativity, logic, and linguistic finesse.

However, while LLMs demonstrate remarkable text generation capabilities, they are devoid of genuine consciousness. Their outputs, although coherent, are statistical reflections of their training data, not indicative of true comprehension. This dichotomy poses intriguing philosophical questions about the essence of thought, creativity, and the intricate dance between human introspection and algorithmic processing. 

==> sections/preamble/acronyms.tex <==
% \acrodef{DL}{deep learning}
% \acrodef{ML}{machine learning}
% \acrodef{NLP}{natural language processing}
% \acrodef{LLM}[LLM]{large language model}
% \acrodef{MLLM}[MLLM]{multimodal large language model}

==> sections/preamble/macros.tex <==
% \newcommand{\ignore}[1]{{}}

% \newcommand{\squishlist}{
% 	\begin{list}{$\bullet$}
% 		{ \setlength{\itemsep}{0pt}
% 			\setlength{\parsep}{1pt}
% 			\setlength{\topsep}{1pt}
% 			\setlength{\partopsep}{0pt}
% 			\setlength{\leftmargin}{0.9em}
% 			\setlength{\labelwidth}{1.5em}
% 			\setlength{\labelsep}{0.4em} } }
% 	\newcommand{\squishend}{
% 	\end{list}  } 
	
	
% \definecolor{graphFirst}{RGB}{2,136,209} % Light Blue 700
% \definecolor{graphSecond}{RGB}{211,47,47} % Red 700
% \definecolor{graphThird}{RGB}{245,124,0} % Orange 700
% \definecolor{graphFourth}{RGB}{56,142,60} % Green 700
% \definecolor{graphFifth}{RGB}{81,45,168} % Deep Purple 700
% \definecolor{graphSixth}{RGB}{69,90,100} % Blue Grey 700
% \definecolor{graphSeventh}{RGB}{251,192,45} % Yellow 700\definecolor{backgroundFirst}{RGB}{129,212,250} % Light Blue 200
% \definecolor{backgroundSecond}{RGB}{239,154,154} % Red 200
% \definecolor{backgroundThird}{RGB}{255,204,128} % Orange 200
% \definecolor{backgroundFourth}{RGB}{165,214,167} % Green 200
% \definecolor{backgroundFifth}{RGB}{179,157,219} % Deep Purple 200
% \definecolor{backgroundSixth}{RGB}{176,190,197} % Blue Grey 200
% \definecolor{backgroundSeventh}{RGB}{255,245,157} % Yellow 200

% \newcommand{\notebox}[2]{\begin{tcolorbox}[enhanced jigsaw,colback=#1,coltext=white,halign=center,sharp corners,boxrule=0pt]#2\end{tcolorbox}}\newcommand{\textDanger}[1]{{\color{graphSecond}#1}}
% \newcommand{\noteDanger}[1]{\notebox{graphSecond}{#1}}\newcommand{\textWarning}[1]{{\color{graphThird}#1}}
% % \newcommand{\noteWarning}[1]{\notebox{graphThird}{#1}}\newcommand{\textInfo}[1]{{\color{graphFirst}#1}}
% \newcommand{\noteInfo}[1]{\notebox{graphFirst}{#1}}\newcommand{\textSuccess}[1]{{\color{graphFourth}#1}}
% \newcommand{\noteSuccess}[1]{\notebox{graphFourth}{#1}}

% \newcommand*{\boxplot}[6]{%
%   \addplot+[
%     line width=.2mm,
%     black,
%     boxplot prepared={
%       lower whisker={#5},
%       lower quartile={#3},
%       median={#2},
%       upper quartile={#4},
%       upper whisker={#6},
%     }
%   ]
%   % No outliers
%   coordinates{};
% }


==> sections/preamble/preamblelistingsconf.tex <==
% \definecolor{mygreen}{rgb}{0,0.6,0}
% \definecolor{mygray}{rgb}{0.5,0.5,0.5}
% \definecolor{mymauve}{rgb}{0.58,0,0.82}

% \makeatletter
% \let\old@lstKV@SwitchCases\lstKV@SwitchCases
% \def\lstKV@SwitchCases#1#2#3{}
% \makeatother
% \usepackage{lstlinebgrd}
% \makeatletter
% \let\lstKV@SwitchCases\old@lstKV@SwitchCases

% \lst@Key{numbers}{none}{%
%     \def\lst@PlaceNumber{\lst@linebgrd}%
%     \lstKV@SwitchCases{#1}%
%     {none:\\%
%      left:\def\lst@PlaceNumber{\llap{\normalfont
%                 \lst@numberstyle{\thelstnumber}\kern\lst@numbersep}\lst@linebgrd}\\%
%      right:\def\lst@PlaceNumber{\rlap{\normalfont
%                 \kern\linewidth \kern\lst@numbersep
%                 \lst@numberstyle{\thelstnumber}}\lst@linebgrd}%
%     }{\PackageError{Listings}{Numbers #1 unknown}\@ehc}}
% \makeatother

% \usepackage{lstlinebgrd} % see http://www.ctan.org/pkg/lstaddons

% \lstset{ 
% %   escapeinside={(*@}{@*)},
% %   backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}; should come as last argument
%   basicstyle=\scriptsize,        % the size of the fonts that are used for the code
% %   breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
%   breaklines=true,                 % sets automatic line breaking
% %   captionpos=b,                    % sets the caption-position to bottom
%   commentstyle=\color{mygreen},    % comment style
% %   deletekeywords={...},            % if you want to delete keywords from the given language
% %   escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
% %   extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
%   frame=single,	                   % adds a frame around the code
% %   keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
%   keywordstyle=\color{blue},       % keyword style
%   language=C,                 % the language of the code
% %   morekeywords={*,...},            % if you want to add more keywords to the set
%   numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
%   numbersep=5pt,                   % how far the line-numbers are from the code
%   numberstyle=\tiny\color{mygray}, % the style that is used for the line-numbers
% %   rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
% %   showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
% %   showstringspaces=false,          % underline spaces within strings only
% %   showtabs=false,                  % show tabs within strings adding particular underscores
% %   stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
%   stringstyle=\color{mymauve},     % string literal style
% %   tabsize=2,	                   % sets default tabsize to 2 spaces
% %   title=\lstname                   % show the filename of files included with \lstinputlisting; also try caption instead of title
% %   %framesep=0pt,framerule=0pt,
% %   %aboveskip=0pt,belowskip=0pt
% }

